CKGAN: Training Generative Adversarial Networks Using Characteristic Kernel Integral Probability Metrics

In this paper, we propose CKGAN, a novel generative adversarial network (GAN) variant based on an integral probability metrics framework with characteristic kernel (CKIPM). CKIPM, as a distance between two probability distributions, is designed to optimize the lowerbound of the maximum mean discrepancy (MMD) in a reproducing kernel Hilbert space, and thus can be used to train GANs. CKGAN mitigates the notorious problem of mode collapse by mapping the generated images back to random noise. To save the effort of selecting the kernel function manually, we propose a soft selection method to automatically learn a characteristic kernel function. The experimental evaluation conducted on a set of synthetic and real image benchmarks (MNIST, CelebA, etc.) demonstrates that CKGAN generally outperforms other MMD-based GANs. The results also show that at the cost of moderately more training time, the automatically selected kernel function delivers very close performance to the best of manually fine-tuned one on real image benchmarks and is able to improve the performances of other MMD-based GANs.

==> proof.tex <==
% Analysis
To make IPM a lower bound of MMD, we need the condition that $\left \| \phi(\cdot) \right \|_\mathcal{H} \leq 1$ in the characteristic kernel. This does not hold for all characteristic kernels. 
See proof in: https://chatgpt.com/share/679e6f07-cd04-8004-9c77-b732756e03b1

In our experiments, RBF mixture does not satisfy this condition. Matern kernels only satisfy this condition when $\alpha \leq 1$ (our setting is $\alpha = 1$). Nonetheless, we can modify the MMD condition by bounding the kernel with a finite constant (e.g., $K = 5$ for the RBF mixture). See: https://chatgpt.com/share/679e88a7-0d24-8004-80fd-ff6a042a5a77

% ChatGPT Prompt
I am designing a generative adversarial network, attempting to jointly use integral probability metrics (IPM) and maximum mean discrepancy (MMD). I have encountered some difficulties when trying to prove a theorem. 

Let $\mathcal{X}$ be a dataset (of images) and $\mathbb{R}^m$ be a vector space. $x$ is a sample drawn from $\mathcal{X}$. 

Let $\mathscr{F}$ be a family of measurable and bounded real valued symmetric (i.e., $\forall f \in \mathscr{F}$, $-f \in \mathscr{F}$) functions on $\mathcal{X}$. Let $\mathscr{P}(\mathcal{X})$ be the set of measurable probability distributions on $\mathcal{X}$. 

Given two probability distributions $\mathbb{P}$, $\mathbb{Q} \in \mathscr{P}(\mathcal{X})$, the integral probability metrics (IPM) indexed by the function space $\mathscr{F}$ is defined as follows: 

$d_\mathscr{F}(\mathbb{P}, \mathbb{Q}) = \underset{f \in \mathscr{F}}{\text{sup}} \left \{  \underset{x\sim \mathbb{P}}{\mathbb{E}} f(x) - \underset{x\sim \mathbb{Q}}{\mathbb{E}} f(x)\right \}$.

The maximum mean discrepancy (MMD) considers $\mathscr{F}$ as the family of functions in the unit ball in a reproducing kernel Hilbert space (RKHS) $\mathcal{H}$ (i.e. $\mathscr{F} := \left \{ f \mid \left \| f \right \|_\mathcal{H} \leq 1\right \}$): 

$MMD(\mathbb{P}, \mathbb{Q}) = \underset{\left \| f \right \|_\mathcal{H}  \leq 1}{\text{sup}} \left \{  \underset{x\sim \mathbb{P}}{\mathbb{E}} f(x) - \underset{x\sim \mathbb{Q}}{\mathbb{E}} f(x)\right \}$. 

A probability distribution $\mathbb{P}$ can be measured by the mean embedding $\mu_\mathbb{P} \in \mathcal{H}$, $\mu_\mathbb{P} = E_{x \sim \mathbb{P}}[\phi(x)]$, where $\phi(\cdot)$ is a feature mapping function that maps to an RKHS $\mathcal{H}$. Given a kernel function $k(x, x') = \langle \phi(x), \phi(x') \rangle_\mathcal{H}$, $k$ is characteristic if and only if $\mathbb{P} \mapsto \mu_\mathbb{P}$ is injective; i.e., $\mathbb{P}$ is mapped to a unique element $\mu_{\mathbb{P}}$ in ${\mathcal{H}}$. 

Now we consider $\mathscr{F}$ as a family of functions having the form $k(z, \Phi_{\omega}(x))$, where $k$ is a characteristic kernel, $z$ is a noise $z$ randomly sampled from a noise set $\mathcal{Z}$ with distribution $\mathbb{P}_z$, and $\Phi_{\omega}$ is a parameterized neural network as a non-linear feature mapping from $\mathcal{X}$ to $\mathbb{R}^m$. Given a characteristic kernel $k(x, x') = \langle \phi(x), \phi(x') \rangle_\mathcal{H}$ satisfying $\left \| \phi(\cdot) \right \|_\mathcal{H} \leq 1$, we consider the following function family: 

$\mathscr{F} := \{ f(x) = \langle \phi(z), \phi (\Phi_{\omega}(x)) \rangle \mid z \in \mathbb{R}^m, \left \| \phi(z) \right \|_\mathcal{H} \leq 1, 
\Phi_{\omega}: \mathcal{X} \rightarrow \mathbb{R}^m, \omega \in \Omega \}$, 

where $\phi(\cdot)$ is a feature mapping function that maps the input to an RKHS $\mathcal{H}$. 

For this $\mathscr{F}$, I want to prove that the IPM $d_\mathscr{F}(\mathbb{P}, \mathbb{Q})$ is a lower bound of the MMD. If not, please tell me the reason. 
